Leveraging Language Models for Analyzing Longitudinal Experiential Data in Education

We propose a novel approach to leveraging pre-trained language models (LMs) for early forecasting of academic trajectories in STEM students using high-dimensional longitudinal experiential data. This data, which captures students' study-related activities, behaviors, and psychological states, offers valuable insights for forecasting-based interventions. Key challenges in handling such data include high rates of missing values, limited dataset size due to costly data collection, and complex temporal variability across modalities. Our approach addresses these issues through a comprehensive data enrichment process, integrating strategies for managing missing values, augmenting data, and embedding task-specific instructions and contextual cues to enhance the models' capacity for learning temporal patterns. Through extensive experiments on a curated student learning dataset, we evaluate both encoder-decoder and decoder-only LMs. While our findings show that LMs effectively integrate data across modalities and exhibit resilience to missing data, they primarily rely on high-level statistical patterns rather than demonstrating a deeper understanding of temporal dynamics. Furthermore, their ability to interpret explicit temporal information remains limited. This work advances educational data science by highlighting both the potential and limitations of LMs in modeling student trajectories for early intervention based on longitudinal experiential data.

==> 5.Related_Work.tex <==
\section{Related Work}
\label{related}
\vspace{-1.00mm}

The research on time-series forecasting by utilizing pre-trained LMs can be broadly divided into two categories~\cite{sun_2023_test}, i.e., model-centric and data-centric. The \textbf{data-centric} approach focuses on converting time-series data by innovating embedding methods to learn suitable representations for the pre-trained LMs. The methods involve embedding solutions to align the text embedding space of LMs with the time-series tokens~\cite{sun_2023_test}, augment embedding by including additional instructions as prompts such as dataset context, task instruction, and input statistics~\cite{jin_2023_timellm}, two-stage fine-tuning approach~\cite{chang_2023_llm4ts}, and a zero-shot approach that focuses on preprocessing the numerical data~\cite{gruver_2023_llm}. The \textbf{model-centric} approach mainly focuses on adapting a pre-trained LM for time-series data by fine-tuning the embedding and normalization layers while keeping self-attention and feedforward layers frozen~\cite{zhou_2023_OFA}, by incorporating additional fine-grained designs such as time series decomposition and soft prompts~\cite{cao_2023_tempo}, formulating forecasting as question answering with prompting~\cite{xue_promptcast_2023}, and prompt-tuning with few-shot learning (prompt engineering)~\cite{liu_2023_llm}.

While we use a model-centric approach to the forecasting problem, unlike the above methods (both data-centric and model-centric), we attempt to solve forecasting problems using experiential data. Also, unlike the soft prompts used in some of the above methods, we use discrete prompts.

